PeerDA: Data Augmentation via Modeling Peer Relation for Span Identification Tasks

Span identification aims at identifying specific text spans from text input and classifying them into pre-defined categories. Different from previous works that merely leverage the Subordinate (SUB) relation (i.e. if a span is an instance of a certain category) to train models, this paper for the first time explores the Peer (PR) relation, which indicates that two spans are instances of the same category and share similar features. Specifically, a novel Peer Data Augmentation (PeerDA) approach is proposed which employs span pairs with the PR relation as the augmentation data for training. PeerDA has two unique advantages: (1) There are a large number of PR span pairs for augmenting the training data. (2) The augmented data can prevent the trained model from over-fitting the superficial span-category mapping by pushing the model to leverage the span semantics. Experimental results on ten datasets over four diverse tasks across seven domains demonstrate the effectiveness of PeerDA. Notably, PeerDA achieves state-of-the-art results on six of them.

==> 2introduction_bak.tex <==
\section{Introduction}
\begin{figure}
    \centering
    \includegraphics[scale=0.19]{intro_example.pdf}
    \caption{(a) Illustrations of Subordinate (\textsc{Sub}) and Peer (\textsc{Pr}) relations in SpanID tasks. (b) The constructions of augmented data with \textsc{Pr} relations in MRC paradigm. We use NER here for demonstration purpose.}
    \label{fig:example}
    \vspace{-11pt}
\end{figure}


Span Identification (SpanID) is a family of Natural Language Processing (NLP) tasks with the goal of detecting specific text spans and further classifying them into pre-defined categories~\cite{papay-etal-2020-dissecting}.
It serves as the initial step for complex text analysis by narrowing down the search scopes of important spans, which holds a pivotal position in the field of NLP~\cite{ding-etal-2021-nerd}.
Recently, different domain-specific SpanID tasks, such as social media Named Entity Recognition (NER) \cite{derczynski-etal-2017-results}, Aspect Based Sentiment Analysis (ABSA) \cite{liu2012sentiment}, Contract Clause Extraction (CCE) \cite{chalkidis2017extracting} and Span Based Propaganda Detection (SBPD) \cite{da-san-martino-etal-2019-fine}, have emerged for various NLP applications.
% However, domain-specific SpanID tasks often suffer from the low-resource\lx{data scarcity?} issue, since they are generally time-consuming and costly to manually annotate sufficient training data for a specific domain\lx{``, since'' ==> because it is generally time-consuming or even impossible to manually annotate sufficient training data for such tasks}.

% Early works \cite{chiu-nichols-2016-named} typically tackle SpanID tasks as a sequence tagging problem, which aims to predict a single label for each input token. 
% Recently, to better exploit the knowledge from pretrained language models \cite{devlin-etal-2019-bert, liu2019roberta}, many efforts \cite{liu-etal-2020-event,yang-etal-2021-enhanced} have been made on reformulating SpanID tasks as a Machine Reading Comprehension (MRC) problem.
% As illustrated in the Figure \ref{fig:example} (b), MRC creates a unique query for each category and solves the SpanID task by extracting corresponding answer spans to the given category queries in the context. 
% Despite such shift of paradigm  \cite{sun2021paradigm}, the primary goal of SpanID remains the same to accurately extracting the \textbf{span-category} Subordinate (\textsc{Sub}) relation --- \textit{if a span is an instance of a certain category}.
% Meanwhile, previous works also make a similar attempt in two paradigms to address the extraction of the \textsc{Sub} relation by intuitively building the training data that reflects the \textsc{Sub} relation.
% More specifically, in sequence tagging, the \textsc{Sub} relation lies in the correct prediction of the category for each input token under certain context. In MRC, the \textsc{Sub} relation is to precisely extract relevant spans given a category query. 
Precisely, as shown in Figure \ref{fig:example} (a), the process of SpanID can be summarized as accurately extracting \textbf{span-category} Subordinate (\textsc{Sub}) relation --- \textit{if a span is an instance of a certain category}.
Early works \cite{chiu-nichols-2016-named} typically tackle SpanID tasks as a sequence tagging problem, where the \textsc{Sub} relation is recognized via predicting the category for each input token under certain context. 
Recently, to better utilize label semantics, many efforts have been made on reformulating SpanID tasks as a Machine Reading Comprehension (MRC) problem \cite{liu-etal-2020-event,yang-etal-2021-enhanced}.
As shown by the example in Figure \ref{fig:example} (b), such formulation first creates a \textsc{Sub} query for each category and then recognizes the \textsc{Sub} relation by detecting relevant spans in the input text (\textit{i.e.}, context) as answers to the category query.

However, only leveraging the \textsc{Sub} relation in the training data to build SpanID models may suffer from two limitations: 
% 1) \textbf{Over-fitting}: With only \textsc{Sub} relation, SpanID models would easily over-fit the superficial span-category mapping on existing categories and show poor generalization to unseen data.
1) \textbf{Over-fitting}: With only \textsc{Sub} relation, SpanID models tend to capture the superficial span-category correlations. Such correlations may misguide the models to ignore the semantics of the given span but make predictions based on the memorized span-category patterns, which hurts the generalization capability of the models.  
% \bingc{这里的unseen data指的是什么？new category么？需要更具体的讨论，什么情况、下为什么overfit。}
% \xww{With only \textsc{Sub} relation, SpanID models are prone to memorizing span-category combinations in the training data, and thus pay less attention to the spans' semantics, resulting in poor generalization to new categories. \bingc{蔚文这里把话说的太绝对，不好但是也没到poor的程度}} \lx{With only \textsc{Sub} relation, SpanID models tend to capture the superficial span-category correlations. Such correlations will encourage the models to ignore the semantics of the given span and its context but make predictions based on the memorized span-category patterns only, which obviously degrade the generalization capability of the models.}
2) \textbf{Data Scarcity}: For low-resource scenarios or long-tailed categories, the number of span-category pairs with \textsc{Sub} relation (\textsc{Sub} pairs) could be very limited and insufficient to learn a reliable SpanID model.

% \bingc{这段对于Pr relation为啥能解决以上两个limitations，讲的不清楚，尤其是对于overfitting的好处。}

In this paper, we explore the \textbf{span-span} Peer (\textsc{Pr}) relation to alleviate the above limitations. Specifically, the \textsc{Pr} relation indicates that \textit{two spans are two different instances of the same category}. 
The major difference is that the \textsc{Pr} relation does not involve the direct supervision signal, \textit{i.e.}, the category information.
For example, in Figure~\ref{fig:example} (a), "Hawaii" and "London" are connected with the \textsc{Pr} relation they are instances of the same category.
% Different from the \textsc{Sub} relation, the strong\xww{direct !} supervision signal, \textit{i.e.}, the category information, is invisible to the \textsc{Pr} relation. 
% With the pretrained contextualized representations \cite{devlin-etal-2019-bert, liu2019roberta}, recognizing the \textsc{Pr} relation allows the two involved spans to share their individual semantic information about their category, which facilitates better span representation learning towards the true semantics of their category.
% \lx{++ \textsc{Pr} relation does not create explicit span-category associations but guides the model to learn task-specific semantic representations that better group the spans belonging to the same category}. 
% Recognizing the \textsc{Pr} relation requires two involved spans to compare their individual semantic information about their category.
% With the pretrained contextualized representations \cite{devlin-etal-2019-bert, liu2019roberta}, this allows one span to fuse additional category information from its peer and thus learns a better span representation, which can enhance the models' capability of capturing the \textsc{Sub} relation.
The number of span-span pairs with the \textsc{Pr} relation (\textsc{Pr} pairs) grows quadratically in the number of \textsc{Sub} pairs.
Therefore, we can still construct a reasonable number of training data with \textsc{Pr} pairs for categories having insufficient examples.
Moreover, the variety of span-span patterns increases the difficulty for the model to make decisions through superficial correlations.
Hence, the model is enforced to weigh more on the span's semantics for recognizing \textsc{Pr} relations.
This advantage also mitigates the above over-fitting issue because the model can leverage the strong semantic understanding capability to recognize the unseen span-category pairs.
% \bingc{一定要注意，claim的点，如果没有实验支撑，不要说的过于绝对，让别人buy in我们的观点，说的太绝对是反效果}

% In this paper, with the aim of leveraging the \textsc{Pr} relation to enhance SpanID models, we propose a Peer Data Augmentation (\textit{PeerDA}) approach that treats \textsc{Pr} pairs as a kind of augmented training data.
% As depicted in Figure~\ref{fig:example} (b), PeerDA is realized in the paradigm of MRC \bingc{应该明确说MRC允许对两类training data进行统一的建模} such that the query can be customized either as a category or a similar span to explore the \textsc{Sub} and \textsc{Pr} relation respectively.
% % Specifically, we extend the usage of the original training data with both the \textsc{Sub} and \textsc{Pr} relation\\textit{i.e.}{Mark} and construct the final training data from both 4\\textit{i.e.}{The training data of PeerDA is constructed from both views of the \textsc{Sub} relation and the \textsc{Pr} relation}:
% To achieve this, we extend the usage of the original training data in two views:
% (1) The \textsc{Sub}-based training data. It directly solves SpanID tasks by extracting the \textsc{Sub} relation in the original training data.
% (2) The \textsc{Pr}-based training data. It is augmented to enrich the semantics of spans by extracting the \textsc{Pr} relation in the original training data, where one span is asked to identify its peer from the context. \bingc{继续写，技术上lijiwei方法有哪些改进。这样显得PeerDA既有方法贡献，也有技术贡献。}


In this paper, with the aim of leveraging the \textsc{Pr} relation to enhance SpanID models, we propose a Peer Data Augmentation (\textit{PeerDA}) approach that treats \textsc{Pr} pairs as a kind of augmented training data.
To achieve this, as depicted in Figure~\ref{fig:example} (b), we extend the usage of the original training data in two views:
(1) The \textsc{Sub}-based training data.  It is used to directly solve the SpanID tasks by extracting the \textsc{Sub} relation in the original training data.
(2) The \textsc{Pr}-based training data. It is augmented to enrich the semantics of spans by extracting the \textsc{Pr} relation in the original training data, where one span is asked to identify its peer from the context.
Both training data are realized in a unified MRC formulation such that the knowledge learned from \textsc{Pr}-based training data can be directly used to enhance the model's capability to capture \textsc{Sub} relation (\textit{i.e.}, solve SpanID tasks).
To better accommodate the MRC-style \textsc{Sub} and \textsc{Pr} data, we develop a stronger and more memory-efficient Multi-Span MRC model (Multi-MRC). Compared to the designs in~\citet{li-etal-2020-unified}, our Multi-MRC model introduces a bilinear component to calculate the span scores (\textit{i.e.}, span-level likelihood) and consistently achieves better results with a 4x smaller memory budget. Besides, we propose a margin-based contrastive learning strategy to additionally model the negative spans regarding the query so that the spans from different categories are separated more apart in the semantic space.


% PeerDA is realized ... => PeerDA unifies the modeling of both \textsc{Sub} and \textsc{Pr} relation in the same MRC formulation by either customizing the query to be a category or a similar span. 
% }


% \bingc{实验部分，需要调整为低资源为主的贡献}
We evaluate the effectiveness of PeerDA on ten datasets across seven domains, from four different SpanID tasks, namely, NER, ABSA, Contract Clause Extraction (CCE), and Span Based Propaganda Detection (SBPD).
Experimental results show that extracting \textsc{Pr} relation benefits the learning of semantics and encourages models to identify more possible spans.
As a result, PeerDA sets new state-of-the-art (SOTA) on six SpanID datasets.
% Experimental results show that extracting \textsc{Pr} relation benefits the learning of semantics and encourages models to identify more possible spans, making it particularly effective on domains or tasks with low tolerance to missing important clues (e.g. legal).\xww{Experimental results ... => As a result, PeerDA sets new state-of-the-art (SOTA) on seven SpanID tasks. }
% We also make diverse analyses to explore more potential scenarios of applying PeerDA.
% \xww{We also... => Our analyses further demonstrates the capability of PeerDA to alleviate scarcity and over-fitting issues.}
Our analyses further demonstrate the capability of PeerDA to alleviate scarcity and over-fitting issues.

Our contributions are summarized as follows:
(1) We propose a novel PeerDA approach to tackle SpanID tasks via augmenting training data with \textsc{Pr} relation.
(2) We conduct extensive experiments on ten datasets, including four different SpanID tasks across seven domains, and achieve SOTA performance on six SpanID tasks.
(3) PeerDA alleviates the scarcity issue, where it is more effective in low-resource scenarios or long-tailed categories. PeerDA also allows models to weigh more on the span semantics, which prevents over-fitting.
% \begin{itemize}[leftmargin=3mm]
% \setlength{\itemsep}{0pt}
% \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
%     \item We propose a novel PeerDA approach to tackle SpanID tasks via augmenting training data with \textsc{Pr} relation.
%     \item We conduct extensive experiments on ten datasets, including four different SpanID tasks across seven domains, and achieve SOTA performance on six SpanID tasks.
%    \item PeerDA alleviates the scarcity issue, where it is more effective in low-resource scenarios or long-tailed categories. PeerDA also allows models to weigh more on the span semantics, which prevents over-fitting.
% \end{itemize}



==> 4method_old.tex <==
\section{SpanID as Multi-Span MRC}
\bingc{如果没有对lijiwei方法的任何改进，显得在技术上没有贡献，审稿人会挑战这一点。需要做一些技术加强。如果没有改进，这部分的篇幅，不应该超过一个column。如果改为短文，应该是半个column。}

MRC is initially designed to only identify one span as the answer to each query, which is not suitable for SpanID that requires identifying multiple spans.
For example, in Figure \ref{fig:multi}, it cannot simultaneously detect the two spans given the query of "Work of Art".
To tackle this issue, we follow the design of \citet{li-etal-2020-unified} to build a Multi-Span MRC model that is capable of simultaneously extracting multiple spans and implement our PeerDA on it. 

\vspace{2pt}
\noindent \textbf{Overview of SpanID:}
Given the input text $X=\{x_1,...,x_n\}$,
SpanID is to detect all important spans $\{x^k_{s,e}\}_{k=1}^K$ and classify them with proper labels $\{y^k\}_{k=1}^K$, where each span $x^k_{s,e}=\{x_{s_k}, x_{s_k+1},...,x_{e_k-1},x_{e_k}\}$ is a continuous subsequence of $X$ satisfying $s_k \le e_k$ and the label comes from a predefined category set $Y$ according to different SpanID tasks (e.g. "Person" in NER).

\vspace{2pt}
\noindent \textbf{Multi-Span MRC:}
The base model consists of three components: an encoder, a span predictor, and a start-end selector. First, given the concatenation of the query $Q$ and the context $X$ as the MRC input $X^{\textrm{MRC}}=\{{\tt [CLS]},Q,{\tt [SEP]},X,{\tt [SEP]}\}$, where ${\tt [CLS]}, {\tt [SEP]}$ are special tokens, the encoder would encode the input text into hidden states $\mathbf{H}^{\textrm{MRC}}$.
\begin{equation}
\setlength{\abovedisplayskip}{5pt}
\setlength{\belowdisplayskip}{1pt}
    \mathbf{H}^{\textrm{MRC}} = \textsc{Encoder}(X^{\textrm{MRC}})
\end{equation}

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{multi-span.pdf}
    \caption{Example of extracting multiple spans in NER.}
    \label{fig:multi}
    \vspace{-10pt}
\end{figure}

Second, the span predictor consists of two binary classifiers, one to predict whether each context token is the start index of the answer based on its hidden state, and the other to predict whether each context token is the end index:
\begin{equation}
\setlength{\abovedisplayskip}{5pt}
\setlength{\belowdisplayskip}{5pt}
\begin{split}
    P_\text{start}&=\textsc{Softmax}(\mathbf{H}^{\textrm{MRC}} \textbf{\textit{W}}^s)\\
    P_\text{end}&=\textsc{Softmax}(\mathbf{H}^{\textrm{MRC}} \textbf{\textit{W}}^e) 
\end{split}
\end{equation}
where $\textbf{\textit{W}}^s,  \textbf{\textit{W}}^e \in \mathbb{R}^{d \times 2}$ are the weights of two classifiers and $d$ is the dimension of hidden states.
The span predictor would output multiple start and end indexes for the given query and context.

Finally, the start-end selector matches each start index to each end index and select the most possible spans from all combinations as the output answers:
\vspace{-5pt}
\begin{equation}
    P_\text{s,e} = \text{sigmoid}(\textbf{\textit{W}}^{sel}[{H}^{\textrm{MRC}}_{s}; {H}^{\textrm{MRC}}_{e}])
\end{equation}
where $P_\text{s,e}$ denotes the probability of $X^{\textrm{MRC}}_{s:e}$ to form a possible answer, $\textbf{\textit{W}}^{sel}  \in \mathbb{R}^{1 \times 2d}$ is the weight matrix and $[;]$ is the concatenation operation.

The overall training objective is to minimize the cross-entropy loss (CE) between three predictions and their corresponding ground-truth labels:
\begin{equation}
\setlength{\abovedisplayskip}{5pt}
\setlength{\belowdisplayskip}{5pt}
\label{eqn:loss}
\begin{split}
    \mathcal{L}=&  \text{CE}(P_\text{start}, Y_\text{start}) + \alpha \text{CE}(P_\text{end}, Y_\text{end}) \\& + \beta \text{CE}(P_\text{s,e}, Y_\text{s,e})
    \end{split}
\end{equation}
where $\alpha, \beta$  and $ Y_\text{start}, Y_\text{end}, Y_\text{s,e}$ are balance rates and golden start, end, and span indices respectively.

\section{PeerDA}
\bingc{如果不增加对lijiwei方法的改进，需要对DA部分，做更多创新。比如增加dissimilar query。}

In this work, we propose a PeerDA approach to perform data augmentation. 
The training data $\mathcal{D}$ consists of two parts:
(1) The \textsc{Sub}-based training data $\mathcal{D^{\textsc{Sub}}}$, where the query is about a category and the MRC context is the input text.
(2) The \textsc{Pr}-based training data $\mathcal{D^{\textsc{Pr}}}$ is constructed with \textsc{Pr} pairs, where one span is used to create the query and the input text containing the second span serves as the MRC context.


\subsection{\textsc{Sub}-based Training Data}
First, we need to transform the original training examples into (query, context, answers) triples following the paradigm of Multi-Span MRC.
To extract the \textsc{Sub} relation between categories and relevant spans, a natural language query $q^{\textsc{Sub}}_y$ is constructed to reflect the semantics of each category $y$.
Following \citet{hendrycks2021cuad}, we include both category mention $\tt [Men]_y$ and its definition $\tt [Def]_y$ from the annotation guideline (or Wikipedia if the guideline is not accessible) in the query to introduce more comprehensive semantics:
\begin{equation}
\begin{aligned}
    q^{\textsc{Sub}}_y=\;&\tt{Highlight\;the\;parts\;(if\;any)}\\
    &\tt{related\;to\;[Men]_y.\;Details:[Def]_y}.
\end{aligned}
\end{equation}

Given the input text $X$ as the context, the answers to $q^{\textsc{Sub}}_y$ are the spans having the category same to $y$.
Then we can obtain one MRC triple denoted as ($q^{\textsc{Sub}}_y$, $X$, $\{x^k_{s,e}\;|\;x^k_{s,e}\in X,y^k=y\}_{k=1}^K$).
By enumerating all categories, we create $|Y|$ training examples for each input text to allow the identification of spans from all categories.

\subsection{ \textsc{Pr}-based training data}
To construct augmented data that explores the \textsc{Pr} relation, we first create a category-wise span set $\mathcal{S}_y$ that includes all training spans with category $y$:
\begin{equation}
    \mathcal{S}_y = \{x^k_{s,e}\; |\; x^k_{s,e} \in \mathcal{D^{\textsc{Sub}}} , y^k = y \}
\end{equation}
Obviously, any two different spans in $\mathcal{S}_y$ have the same category and shall hold the \textsc{Pr} relation.
Therefore, we pair every two different spans in $\mathcal{S}_y$ to create a peer set $\mathcal{P}_y$:
\begin{equation}
    \mathcal{P}_y = \{(x^q_{s,e},x^a_{s,e})\; |\; x^q_{s,e},x^a_{s,e} \in \mathcal{S}_y ,\\ x^q_{s,e} \ne x^a_{s,e} \}
\end{equation}

For each \textsc{Pr} pair in $\mathcal{P}_y$, we can construct one training example by constructing the query with the first span $x^q_{s,e}$:
\begin{equation}
\begin{aligned}
    q^{\textsc{Pr}}_y=\;&\tt{Highlight\;the\;parts\;(if\;any)\;} \\
    & \tt{similar\;to\;}\mathit{x^q_{s,e}}.
\end{aligned}
\end{equation}
Then the text $X^a$ containing the second span $x^a_{s,e}$ denotes the MRC context, and the spans having the same category $y$ in $X^a$ are the answers. Finally, we obtain the MRC triple with respect to the \textsc{Pr} relation as ($q^{\textsc{Pr}}_y$, $X^a$, $\{x^k_{s,e}\;|\;x^k_{s,e}\in X^a,y^k=y\}_{k=1}^K$).

Theoretically, given the span set $\mathcal{S}_y$, there are only $|\mathcal{S}_y|$ \textsc{Sub} pairs in the training data but we can obtain $|\mathcal{S}_y| \times (|\mathcal{S}_y| - 1)$ \textsc{Pr} pairs to construct $\mathcal{D^{\textsc{Pr}}}$.
% Such large size\lx{==> number?} of augmented data may not always be beneficial because 
% (1) the high-resource category labels get more \textsc{Pr} relations, which makes the data distribution more skewed; 
% (2) the performance of SpanID is not always positively correlated with the size of indirect training data (i.e. \textsc{Pr}). 
% Therefore, we propose three augmentation strategies to control the size and distribution of augmented data\lx{Note: the abundance of the augmented data is an advantage of Pr-based DA but here you directly present its disadvantage}.
Such a large number of augmented data shall hold great potential to enrich spans' semantics. 
However, putting all \textsc{Pr}-based examples into training would make the data distribution more skewed since the long-tailed categories get less \textsc{Pr} pairs for augmentation and also increase the training cost.
Therefore, as the first step for DA with the \textsc{Pr} relation, we propose three augmentation strategies to control the size and distribution of augmented data.
We leave more advanced augmentation strategies in future work.

\vspace{4pt}
\noindent \textbf{PeerDA-Size:}
This is to increase the size of augmented data while keeping the data distribution unchanged.
Specifically, for each category $y$, we randomly sample $\lambda|\mathcal{S}_y|$ \textsc{Pr} pairs from $\mathcal{P}_y$. Then we collect all sampled \textsc{Pr} pairs to construct $\mathcal{D^{\textsc{Pr}}}$, where $\lambda$ is the DA rate to control the size of $\mathcal{D^{\textsc{Pr}}}$.

\vspace{4pt}
\noindent \textbf{PeerDA-Categ:}
Categories are not evenly distributed in the training data, and in general SpanID models perform poorly on long-tailed categories because of the insufficient learning of semantics from a limited number of \textsc{Sub} pairs.
To tackle this issue, we propose a PeerDA-Categ strategy to augment more training data for long-tailed categories.
Specifically, let $y^*$ denote the category having the largest span set with the size of $|\mathcal{S}_{y^*}|$. We randomly sample $|\mathcal{S}_{y^*}| - |\mathcal{S}_y|$ \textsc{Pr} pairs from $\mathcal{P}_y$ for each category $y$ and construct a category-balanced training set $\mathcal{D^{\textsc{Pr}}}$ using all sampled pairs. Theoretically, we would get the same size of the training data for each category after the augmentation, which significantly increases the exposure for spans from the long-tailed categories.

\vspace{4pt}
\noindent \textbf{PeerDA-Both:}
To take advantage of the above two strategies, we further propose PeerDA-Both, which allows to maintain the data distribution and, at the same time, effectively increase the size of training data. In PeerDA-Both, we randomly sample $\max( \lambda|\mathcal{S}_{y^*}| + (|\mathcal{S}_{y^*}| - |\mathcal{S}_y|),0)$ \textsc{Pr} pairs from $\mathcal{P}_y$ for each category $y$ to construct $\mathcal{D^{\textsc{Pr}}}$, where $\lambda|\mathcal{S}_{y^*}|$ is to control the size and $|\mathcal{S}_{y^*}| - |\mathcal{S}_y|$ is to control the data distribution.
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{@{}l||p{13mm}<{\centering}p{11mm}<{\centering}p{7mm}<{\centering}p{12mm}<{\centering}cccccc@{}}\toprule
        Task  &  \multicolumn{5}{c}{NER} & \multicolumn{2}{c}{ABSA}  & CCE & \multicolumn{2}{c}{SBPD}\\ 
                 \cmidrule(lr){1-1}\cmidrule(lr){2-6}\cmidrule(lr){7-8}\cmidrule(lr){9-9}\cmidrule(lr){10-11}
        Dataset & \textbf{OntoNotes5}  & \textbf{WNUT17} & \textbf{Movie} & \textbf{Restaurant} & \textbf{Weibo} & \textbf{Lap14}  & \textbf{Rest14} & \textbf{CUAD} & \textbf{News20} & \textbf{Social21}\\ 
        Domain & \textit{mixed}  & \textit{social} & \textit{movie} & \textit{restaurant} & \textit{social} & \textit{laptop}  & \textit{restaurant} & \textit{legal} & \textit{news} & \textit{social} \\ 
        \# Train    & 60.0k  & 3.4k & 7.8k & 7.7k & 1.3k & 2.7k   & 2.7k    & 0.5k & 0.4k     & 0.7k\\ 
        \# Test     & 8.3k  & 1.3k & 2.0k & 1.5k &  0.3k & 0.8k   & 0.8k    & 0.1k & 75 (\textit{dev}) & 0.2k\\
        \# Category & 11     & 6    & 12   & 8 &  4    & 1 / 3  &  1 / 3  & 41   &14        & 20 \\ \bottomrule
    \end{tabular}
    \caption{Statistics on the ten SpanID datasets. Note that 1 / 3 denotes that there is 1 category in ATE and 3 categories in UABSA. \textit{dev} denotes that we evaluate News20 on the dev set.}
    \label{tab:statis}
    \vspace{-10pt}
\end{table*}
\subsection{Train}
We combine the $\mathcal{D^{\textsc{Sub}}}$ and $\mathcal{D^{\textsc{Pr}}}$ constructed above to obtain the final training data.
However, an input text is unlikely to contain all kinds of categories. When converting the text into the MRC paradigm, many of the $|Y|$ examples are unanswerable. If a SpanID model is trained on this unbalanced data, it is likely to output an empty span since it has been taught by the unanswerable examples not to extract spans. 
To mitigate such imbalance, we follow \citet{hendrycks2021cuad} to randomly clear away some unanswerable examples from the training data, such that answerable and unanswerable examples are approximately balanced. 



==> introduction-bak.tex <==
\section{Introduction}
\begin{figure}
    \centering
    \includegraphics[scale=0.19]{intro_example.pdf}
    \caption{(a) Illustrations of Belonging (\textsc{Bl}) and Matching (\textsc{Mc}) relations in SpanID tasks. (b) The constructions of augmented data with \textsc{Mc} relations in MRC paradigm. We use NER here for demonstration purpose.}
    \label{fig:example}
\end{figure}

Span Identification (SpanID) is a family of fundamental Nature Language Processing (NLP) tasks that requires models to detect a small portion of continuous spans and further classify them into relevant category labels~\cite{papay-etal-2020-dissecting}. For example, Named Entity Recognition (NER) is the most famous SpanID task~\cite{nadeau2007survey}. 
SpanID tasks usually serve as the initial step for further complex text analysis by narrowing down the search scopes of important spans, which hold a pivotal position in the field of NLP~\cite{ding-etal-2021-nerd}.
Recently, many domain-specific SpanID tasks, such as social media NER~\cite{derczynski-etal-2017-results}, Aspect Based Sentiment Analysis (ABSA)~\cite{liu2012sentiment}, and Contract Clause Extraction (CCE)~\cite{chalkidis2017extracting}, have emerged due to increasing demands in many NLP applications.
Typically, the high performance of these tasks relies on the availability of large-scale high-quality training data.
However, annotating such data usually requires domain expert knowledge (e.g. legal) and the data may quickly become outdated (e.g. social media) due to the rapid change of language, leaving the annotation cost unaffordable~\cite{chen2021data}.

Data Augmentation (DA) is a widely-adopted solution to the data scarcity issue. Since the primary goal of SpanID model is to accurately recognizing the span-category Belonging (\textsc{Bl}) relation --- \textit{if a span belongs to a certain category}, the existing DA approaches in the context of SpanID mainly attempt to enhance the SpanID model by introducing plenty of previously unseen but meaningful \textsc{Bl}\lx{==>Note: not sure if we should say ``span-category patterns'' for clarity} patterns. Several strategies, such as Span Replacement \cite{dai-adel-2020-analysis,zhou2021melm}, Self-training \cite{xie2020self,liu-etal-2021-machine}, and Distantly Supervised Training \cite{jain-etal-2019-entity, huang-etal-2021-shot} have been proposed to achieve the augmentation of \textsc{Bl} patterns and obtain encouraging results.

% In fact, SpanID tasks are to capture all label-span Belonging (\textsc{Bl}) relations --- \textit{if a span belongs to a certain category}. Considering the example from Figure~\ref{fig:example}, there is only one \textsc{Bl} relation under current context, namely "LOC"-"London".
% Existing Data Augmentation (DA) approaches for SpanID, though are different in terms of methodologies, such as Span Replacement \cite{wei-zou-2019-eda}, Self-Training \cite{xie2019unsupervised,xie2020self}, and Distantly Supervised Training \cite{jain-etal-2019-entity, huang-etal-2021-shot}, they
% only construct task-consistent data that has the same usage as existing training data to explore more \textsc{Bl} relations that have not been seen before.

% Despite their differences, the augmented data from existing approaches are task-consistent, where they follow the same motivation and formalization as the original training data to predict a category label for a span. Such  can be summarized to capturing the Belonging (\textsc{Bl}) relations --- \textit{if a span belongs to a certain category}.
% both the augmented data and original training data are used identically to predict a category label for a span, which can be summarized to enhance the modeling of Belonging (\textsc{Bl}) relations --- \textit{if a span belongs to a certain category}.
%  As shown in Figure~\ref{}, \textsc{Bl} lies in the correct classification of the span in the paradigm of sequence tagging, while in the paradigm of machine reading comprehension (MRC), it lies in the semantic entailment between the span and query category.
\lx{Note: another problem is that the \textsc{Mc}-based augmentation is not straightforward and need special design in terms of the task formulation. Do we need to mention the MRC formulation in the first paragraph?} 

\lx{Present the difference between \textsc{Bl} and \textsc{Mc}. Demonstrate that why exploiting \textsc{Mc} relations is promising (without mentioning DA works).}

On the other hand, as shown in Figure~\ref{fig:example}, the diverse span-span Matching (\textsc{Mc}) relations, which capture the common characteristics or semantics of spans coming from the same category, are largely ignored in the existing DA works. Different from \textsc{Bl} relations, \textsc{Mc} relations do not explicitly associate a span with some categories/labels\lx{==> some category/label but create semantic interaction between arbitrary span pairs within the same category}, which cannot be directly used to solve SpanID tasks.
However, since \textsc{Mc} relations involve spans only from the same category, they are capable to enrich the semantics of an augmented span by fusing the category-related information from its peers and thus encourage it to infer its category.\lx{``, which cannot..''==>. Although \textsc{Mc} relations cannot be used directly as the supervision of training spanID model, they are capable to enrich the semantics of an augmented span by fusing the category-related information from its peers and thus encourage it to infer its category.}
Therefore, from the viewpoint of crafting augmented training samples, DA with \textsc{Mc} relations has two unique advantages over the previous \textsc{Bl}-based DA works: 
First, the candidate set of \textsc{Mc} relations grows quadratically in category size and thus the \textsc{Mc}-based augmentation is able to create a large number of meaningful examples that can enrich spans' semantics. This is extremely beneficial to some low-resource spans because capturing more \textsc{Bl} relations about them is rather difficult due to their scarcity, while we can still construct a relatively large size of \textsc{Mc}-based training data at a low cost. \lx{Second, \textsc{Mc} relations does not introduce pseudo-labeled data}
Second, jointly capturing both \textsc{Bl} and \textsc{Mc} relations allows the SpanID model to pay more attention to the spans' semantics instead of overfitting to the superficial span-label mapping, which is a severe problem of neural network models~\cite{jia-liang-2017-adversarial}.
% Intuitively, \textsc{Mc}-based augmentation suffers less from augmentation noise because \textsc{Mc} relation does not explicitly associate an augmented span with the some category/label but encourage the augmented span to infer the category via semantic matching with other spans of the same category.

Our motivation is borrowed from the legal system, where countries around the world generally follow two practices: the civil law system and the common law system. In civil law systems, judicial decisions are drawn from codified statutes based on the \textsc{Bl} relation between the case and statutes, whereas in common law systems, decisions rely on learning \textsc{Mc} relations from published judicial cases.
Though different in practice, the two systems lead to the same goal of justice and it has been reported that the two systems are mutually beneficial~\cite{pejovic2001civil}.

In this paper, we propose a novel DA approach, namely \emph{MatchDA}, for SpanID tasks from the perspective of capturing \textsc{Mc} relations. 
To enhance the model training using both of the \textsc{Bl} and \textsc{Mc} relations, MatchDA follows the paradigm of machine reading comprehension (MRC), where SpanID tasks can be characterized as extracting spans in a context according to some queries~\cite{li-etal-2020-unified,liu-etal-2020-event} and we are able to customize the queries either as a category label or a similar span to capture the \textsc{Bl} and \textsc{Mc} relations respectively.
Specifically, our entire training data consist of two parts: 
(1) The \textsc{Bl}-based training data, which is converted from the original training data to solve SpanID tasks. It captures \textsc{Bl} relations between a span and its associated category;
(2) The \textsc{Mc}-based training data, which is newly augmented to enrich the semantics of spans. It captures \textsc{Mc} relations by pairing two spans from the same category, where one span is allowed to learn from the other.

We evaluate the effectiveness of MatchDA on nine datasets, including four different SpanID tasks across six domains. The experimental results show that \textsc{Mc} relations enrich the spans with strong semantics and allow models to identify more possible spans, which favors domains or tasks having lower tolerance to missing important clues (e.g. legal).
We also explore SpanID tasks in the context of few-shot transfer and low-resource scenarios to bring more valuable insights of our approach.

To summarize, our contributions are summarized as followed:
\begin{itemize}[leftmargin=4mm]
    \item We provide a novel MatchDA approach for SpanID tasks from the perspective of capturing \textsc{Mc} relations.
    \item We conduct extensive experiments on nine datasets, including four different SpanID tasks across six domains, and show the overall effectiveness of our approach.
    \item We conduct analysis in detail to find when and how to better use our MatchDA.
\end{itemize}
